Accurate Retraining-free Pruning for Pretrained Encoder-based Language Models

Given a pretrained encoder-based language model, how can we accurately compress it without retraining? Retraining-free structured pruning algorithms are crucial in pretrained language model compression due to their significantly reduced pruning cost and capability to prune large language models. However, existing retraining-free algorithms encounter severe accuracy degradation, as they fail to handle pruning errors, especially at high compression rates. In this paper, we propose K-prune (Knowledge-preserving pruning), an accurate retraining-free structured pruning algorithm for pretrained encoder-based language models. K-prune focuses on preserving the useful knowledge of the pretrained model to minimize pruning errors through a carefully designed iterative pruning process composed of knowledge measurement, knowledge-preserving mask search, and knowledge-preserving weight-tuning. As a result, K-prune shows significant accuracy improvements up to 58.02%p higher F1 score compared to existing retraining-free pruning algorithms under a high compression rate of 80% on the SQuAD benchmark without any retraining process.

==> 088reproduce.tex <==
%\mybf{Reproducibility}
%We attach the source code of \method in the supplementary material for reproducibility. We provide detailed experimental settings including hyperparameters in Section~\ref{subsec:setup}, and sensitivity analysis results for three hyperparameters in Appendix~\ref{app:obs}. 
